Enforcing connectivity of 3D linear structures using their 2D projections

Many biological and medical tasks require the delineation of 3D curvilinear structures such as blood vessels and neurites from image volumes. This is typically done using neural networks trained by minimizing voxel-wise loss functions that do not capture the topological properties of these structures. As a result, the connectivity of the recovered structures is often wrong, which lessens their usefulness. In this paper, we propose to improve the 3D connectivity of our results by minimizing a sum of topology-aware losses on their 2D projections. This suffices to increase the accuracy and to reduce the annotation effort required to provide the required annotated training data. Code is available at https://github.com/doruk-oner/ConnectivityOnProjections.

==> fig/fig_boxplot.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[hbt!]
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabular}{c c c}
	\includegraphics[width=0.32\textwidth]{fig/qual_box2}&
	\includegraphics[width=0.32\textwidth]{fig/apls_box2} &
	\includegraphics[width=0.32\textwidth]{fig/tlts_box2} \\
	(a) & (b) & (c)
\end{tabular}
% \vspace{-4mm}
\caption{Median and quartiles over five training runs of scores attained by networks trained with different loss functions. Minimizing our topology-aware loss results in significantly higher score values than minimizing hte baselines. }
\label{fig_boxplot}
\end{figure*}




==> fig/fig_boxplot_mra.tex <==
% !TEX root = ../supplement.tex
% !TEX spellcheck = en-US

\begin{figure*}[hbt!]
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabular}{c c c}
	\includegraphics[width=0.32\textwidth]{fig/qual_box_mra}&
	\includegraphics[width=0.32\textwidth]{fig/apls_box_mra} &
	\includegraphics[width=0.32\textwidth]{fig/tlts_box_mra} \\
	(a) & (b) & (c)
\end{tabular}
% \vspace{-4mm}
\caption{Median and quartiles over five training runs of scores attained by networks trained with different loss functions on \bmra{} dataset. Minimizing our topology-aware loss results in significantly higher score values than minimizing the baselines. }
\label{fig_boxplot_mra}
\end{figure*}




==> fig/fig_boxplot_tabea.tex <==
% !TEX root = ../supplement.tex
% !TEX spellcheck = en-US

\begin{figure*}[hbt!]
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabular}{c c c}
	\includegraphics[width=0.32\textwidth]{fig/qual_box_tabea}&
	\includegraphics[width=0.32\textwidth]{fig/apls_box_tabea} &
	\includegraphics[width=0.32\textwidth]{fig/tlts_box_tabea} \\
	(a) & (b) & (c)
\end{tabular}
% \vspace{-4mm}
\caption{Median and quartiles over five training runs of scores attained by networks trained with different loss functions on \bneuronsmisal{} dataset. Minimizing our topology-aware loss results in significantly higher score values than minimizing the baselines. }
\label{fig_boxplot_tabea}
\end{figure*}




==> tab/results_alpha.tex <==
% !TEX root = ../supplement.tex
% !TEX spellcheck = en-US

\begin{table}[h]
	\centering
	\caption{
		We varied $\alpha$ to investigate its impact on the test performance in \bneurons{} dataset.
		The results show that setting this coefficient too-low or too-high perturbed performance, and its optimal value is in the order of $1e-3$.
		\label{tab:results_alpha}
	}
	% \vspace{5mm}
	\setlength{\tabcolsep}{5pt}
	\begin{tabular}{@{} l l c c   c   c  c  c@{} }
		\toprule
		&& \multicolumn{3}{c}{Pixel-wise} & &  \multicolumn{2}{c}{Topology-aware}\\
		\cmidrule{3-5}
		\cmidrule{7-8}
		
		
		$\alpha$  &  $\beta$  &     
		Corr. &      Comp. &       Qual.  &  &      APLS &        TLTS \\
		\midrule
		
		1e-2 & \multirow{3}{*}{0.1} &
		88.2 &        {\bf 97.0} &     85.9 &   &     74.7 &    85.3    \\ 
		1e-3 & &
		{\bf 98.3} & 96.7 &{\bf 95.1} & & {\bf 87.1} &{\bf 89.6} \\
		1e-4 & &
		98.1 &        96.0 &        94.3 &   &     81.8 &    87.7    \\ 
		\bottomrule
	\end{tabular}
\end{table}



==> tab/results_beta.tex <==
% !TEX root = ../supplement.tex
% !TEX spellcheck = en-US

\begin{table}[h]
	\centering
	\caption{
		We varied $\beta$ to investigate its impact on the test performance in \bneurons{} dataset.
		According to all the performance measures, the best results are obtained for $\beta=0.1$.
		\label{tab:results_beta}
	}
	\setlength{\tabcolsep}{5pt}
	% \vspace{5mm}
	\begin{tabular}{@{} l l c c   c   c  c  c@{} }
		\toprule
		&& \multicolumn{3}{c}{Pixel-wise} & &  \multicolumn{2}{c}{Topology-aware}\\
		\cmidrule{3-5}
		\cmidrule{7-8}
		
		
		$\alpha$  &  $\beta$  &     
		Corr. &      Comp. &       Qual.  &  &      APLS &        TLTS \\
		\midrule
		\multirow{3}{*}{1e-3}
		& 1 &
		 96.3 &  96.4 &     92.9 &   &  85.7    &       87.5 \\ 
		&0.1&
		{\bf 98.3} & 96.7 &{\bf 95.1} & & {\bf 87.1} &{\bf 89.6} \\ 
		& 0.01 &
		95.9 &        {\bf 96.9} &        93.1 &   &     85.3 &    88.9    \\ 
		\bottomrule
	\end{tabular}
\end{table}



==> tab/timing.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}[t]
	\centering
	\caption{
		Time needed to annotate 14 volumes of 250x250x200. The result of user study conducted in~\cite{Kozinski18}.
		\label{tab:timing}
	}
	\setlength{\tabcolsep}{5pt}
	\begin{tabular}{@{} l  c c @{} }
		\toprule
		Annotation type &     Annotation time (mins) &       \% of 3D time.  \\
		\midrule
		Annotating in 3D & 609 & 100 \\
		Annotating in 3 2D MIPs & 387 & 64 \\
		\bottomrule
	\end{tabular}
\end{table}


